Search for SUSY and Higgs particles

An overview of hints for new physics outside the Standard Model and the status of sparticle and Higgs searches is given. The present limits on Higgs bosons of about 90 GeV as well as the $\bsg$ rate and cosmological constraints severely restrict the available parameter space of the MSSM.

==> susy_2e.tex <==
% SUSY Particle names
%auto-ignore
\newcommand{\cha}{\ensuremath{\widetilde{\chi}}}
\newcommand{\chiz}{\ensuremath{\tilde{\chi}^0}}
\newcommand{\chip}{\ensuremath{\chi'}}
\newcommand{\chipp}{\ensuremath{\chi''}}
\newcommand{\chippp}{\ensuremath{\chi'''}}
\newcommand{\sferm}{\ensuremath{\tilde{\mathrm f}}}
\newcommand{\sq}{\ensuremath{\tilde{\mathrm q}}}
\newcommand{\sg}{\ensuremath{\tilde{\mathrm g}}}
\newcommand{\sgrav}{\ensuremath{\tilde{\mathrm G}}}
\newcommand{\snu}{\ensuremath{\tilde{\nu}}}
\newcommand{\snue}{\ensuremath{\tilde{\mathrm{\nu_e}}}}
\newcommand{\snumu}{\ensuremath{\tilde{\nu_\mu}}}
\newcommand{\snutau}{\ensuremath{\tilde{\nu_\tau}}}
\newcommand{\snubar}{\ensuremath{\overline{\nu}}}
\newcommand{\nubar}{\ensuremath{\overline{\nu}}}
\newcommand{\slep}{\ensuremath{\tilde{\ell}}}
\newcommand{\se}{\ensuremath{\tilde{\mathrm{e}}}}
\newcommand{\smu}{\ensuremath{\tilde{\mu}}}
\newcommand{\stau}{\ensuremath{\tilde{\tau}}}
\newcommand{\sw}{\ensuremath{\mathrm{\widetilde{W}}}}
\newcommand{\sz}{\ensuremath{\mathrm{\widetilde{Z}}}}
\newcommand{\sga}{\ensuremath{\mathrm{\widetilde{\gamma}}}}
\newcommand{\sdq}{\ensuremath{\mathrm{\tilde{d}}}}
\newcommand{\suq}{\ensuremath{\mathrm{\tilde{u}}}}
\newcommand{\ssq}{\ensuremath{\mathrm{\tilde{s}}}}
\newcommand{\scq}{\ensuremath{\mathrm{\tilde{c}}}}
\newcommand{\sbq}{\ensuremath{\mathrm{\tilde{b}}}}
\newcommand{\stq}{\ensuremath{\mathrm{\tilde{t}}}}
\newcommand{\sdqbar}{\ensuremath{\mathrm{\overline{\tilde{d}}}}}
\newcommand{\suqbar}{\ensuremath{\mathrm{\overline{\tilde{u}}}}}
\newcommand{\ssqbar}{\ensuremath{\mathrm{\overline{\tilde{s}}}}}
\newcommand{\scqbar}{\ensuremath{\mathrm{\overline{\tilde{c}}}}}
\newcommand{\sbqbar}{\ensuremath{\mathrm{\overline{\tilde{b}}}}}
\newcommand{\stqbar}{\ensuremath{\mathrm{\overline{\tilde{t}}}}}
% parameters
\newcommand{\tb}{\ensuremath{\tan\beta}}
\newcommand{\sqtw}{\ensuremath{\sin^2\Theta_W}}
% RPV
\newcommand{\rpv}{\ensuremath{\mathrm{\not \!\! R_p}}}
\newcommand{\llnu}{\ensuremath{\mathrm{ll\nu}}}
\newcommand{\Hbar}{{\bar H}}
\newcommand{\Ubar}{{\bar U}}
\newcommand{\Dbar}{{\bar D}}
\newcommand{\Ebar}{{\bar E}}
\newcommand{\lle}[3]{\ensuremath{L_{#1}L_{#2}\Ebar_{#3}}}
\newcommand{\lqd}[3]{\ensuremath{L_{#1}Q_{#2}\Dbar_{#3}}}
\newcommand{\udd}[3]{\ensuremath{\Ubar_{#1}\Dbar_{#2}\Dbar_{#3}}}
% variables
\newcommand{\emiss}{\ensuremath{\not \!\! E}}
\newcommand{\etmiss}{\ensuremath{\not \!\! E_t}}
%\newcommand{\ptmiss}{\ensuremath{\not \!\! P _t}}
\newcommand{\rpviol}{\ensuremath{\not \!\! R _P}}
\newcommand{\dm}{\ensuremath{\Delta M}}
% misc
\newcommand{\nbarnf}{\ensuremath{\overline{N_{95}}}}

